EHR-SeqSQL : A Sequential Text-to-SQL Dataset For Interactively Exploring Electronic Health Records

In this paper, we introduce EHR-SeqSQL, a novel sequential text-to-SQL dataset for Electronic Health Record (EHR) databases. EHR-SeqSQL is designed to address critical yet underexplored aspects in text-to-SQL parsing: interactivity, compositionality, and efficiency. To the best of our knowledge, EHR-SeqSQL is not only the largest but also the first medical text-to-SQL dataset benchmark to include sequential and contextual questions. We provide a data split and the new test set designed to assess compositional generalization ability. Our experiments demonstrate the superiority of a multi-turn approach over a single-turn approach in learning compositionality. Additionally, our dataset integrates specially crafted tokens into SQL queries to improve execution efficiency. With EHR-SeqSQL, we aim to bridge the gap between practical needs and academic research in the text-to-SQL domain. EHR-SeqSQL is available at https://github.com/seonhee99/EHR-SeqSQL.

==> tables/compositional_split.tex <==

\begin{table*}[h!]
\centering
\begin{tabular}{ll|l}
\hline
\multicolumn{2}{c|}{\textbf{Split}}                                  & \multicolumn{1}{c}{\textbf{Question}}                                                                                                                                                       \\ \hline
\multicolumn{1}{l|}{\multirow{2}{*}{Compositional}} & Train & \begin{tabular}[c]{@{}l@{}}Count the number of current patients aged 20s.\\ What is the name of insurance of patient 42353 last year?\end{tabular} \\ \cline{2-3} 
\multicolumn{1}{l|}{}                               & Test  & What is the age of patient 53543 in 2013?                                                                                                                      \\ \hline
\end{tabular}
\caption{\label{tab:composition_ex}
An example of data composition in the compositional split.
}
\end{table*}

==> tables/execution_time.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t!]
\small
\renewcommand{\arraystretch}{1.3}
\begin{minipage}{.3\linewidth}
\begin{tabular}{c|c|cc|cc}
\hline
\multirow{2}{*}{\textbf{\# Patient}} & \multirow{2}{*}{\textbf{ST}} & \multicolumn{2}{c|}{\textbf{SQL}} & \multicolumn{2}{c}{\textbf{SQL${^\dag}$}} \\ \cline{3-6} 
& & \multicolumn{1}{c|}{avg.↓}   & med.↓  & \multicolumn{1}{c|}{avg.↓}      & med.↓     \\ \hline
\renewcommand{\arraystretch}{1}

\multirow{2}{*}{\textbf{1k}} & \multicolumn{1}{|c|}{O}  & \multicolumn{1}{c|}{0.20}     & 0.09 & \multicolumn{1}{c|}{\textbf{0.09}}  & \textbf{0.01}       \\ \cline{2-6}

& \multicolumn{1}{|c|}{X}  & \multicolumn{1}{c|}{0.226}   & 0.003   & \multicolumn{1}{c|}{\textbf{0.224}} & 0.003  \\ \hline
\multirow{2}{*}{\textbf{10k}} & \multicolumn{1}{|c|}{O} & \multicolumn{1}{c|}{3.248}  & 1.167 & \multicolumn{1}{c|}{\textbf{1.15}}  &  \textbf{0.15}  \\ \cline{2-6}
& \multicolumn{1}{|c|}{X} & \multicolumn{1}{c|}{11.54} & \multicolumn{1}{c|}{0.013} & \multicolumn{1}{c|}{\textbf{\textbf{10.94}}} & 0.013 \\ \hline
\multirow{2}{*}{\textbf{46k}} & \multicolumn{1}{|c|}{O} & \multicolumn{1}{c|}{31.57}    & 4.60  & \multicolumn{1}{c|}{\textbf{6.00}}  & \textbf{0.52} \\\cline{2-6}
& \multicolumn{1}{|c|}{X}  & \multicolumn{1}{c|}{225.47}  & \multicolumn{1}{c|}{0.076}  & \multicolumn{1}{c|}{\textbf{205.52}}  & \textbf{0.063}
\\ \hline
\end{tabular}
\end{minipage} 
\caption{\label{Exp2.2}
Execution time of SQL queries in the databases with different sizes in terms of the average and median. The time is measured in deciseconds ($10^{-1}$).
}
\end{table}

==> tables/split_stat.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[t!]
\small
\renewcommand{\arraystretch}{1.2}
\begin{minipage}{.2\linewidth}
\begin{tabular}{c|cc|cc}
\hline
\multirow{2}{*}{\textbf{Split}}                                                    & \multicolumn{2}{c|}{\textbf{Random}} & \multicolumn{2}{c}{\textbf{Compositional}} \\ \cline{2-5} 
                                                                                   & \multicolumn{1}{c|}{Train}   & Test  & \multicolumn{1}{c|}{Train}      & Test     \\ \hline
\renewcommand{\arraystretch}{1}
\# of Question Temp                                                           & \multicolumn{1}{c|}{167}     & 166   & \multicolumn{1}{c|}{121}        & 46       \\ 
\# of Interactions                                                                   & \multicolumn{1}{c|}{8,546}   & 649   & \multicolumn{1}{c|}{6,375}      & 2,820    \\ 
\# of Turns                                                                         & \multicolumn{1}{c|}{29,438}  & 2,231 & \multicolumn{1}{c|}{22,134}     & 9,535    \\ 
\begin{tabular}[c]{@{}c@{}}Avg. \# of Turns\end{tabular} & \multicolumn{1}{c|}{3.44}    & 3.44  & \multicolumn{1}{c|}{3.47}       & 3.38     \\ \hline
\end{tabular}
\end{minipage} 
\caption{\label{tab:split_stat}
Statistics for two different splits.}
\end{table}
